Improving Bandwidth Efficiency in E-band Communication Systems

The allocation of a large amount of bandwidth by regulating bodies in the 70/80 GHz band, i.e., the E-band, has opened up new potentials and challenges for providing affordable and reliable Gigabit per second wireless point-to-point links. This article first reviews the available bandwidth and licensing regulations in the E-band. Subsequently, different propagation models, e.g., the ITU-R and Cane models, are compared against measurement results and it is concluded that to meet specific availability requirements, E-band wireless systems may need to be designed with larger fade margins compared to microwave systems. A similar comparison is carried out between measurements and models for oscillator phase noise. It is confirmed that phase noise characteristics, that are neglected by the models used for narrowband systems, need to be taken into account for the wideband systems deployed in the E-band. Next, a new multi-input multi-output (MIMO) transceiver design, termed continuous aperture phased (CAP)-MIMO, is presented. Simulations show that CAP-MIMO enables E-band systems to achieve fiber-optic like throughputs. Finally, it is argued that full-duplex relaying can be used to greatly enhance the coverage of E-band systems without sacrificing throughput, thus, facilitating their application in establishing the backhaul of heterogeneous networks.

==> CRLB3.tex <==
\vspace*{-4pt}
\section{Improving Bandwidth Efficiency in E-band}\label{sec:challenges}

\subsection{LoS MIMO in E-band}\label{sec:eband-MIMO}

\textbf{MIMO in E-band:} It is well-know that application of MIMO in LoS point-to-point wireless systems is challenging because of the large antenna spacing and the fact that different oscillators need to be placed at each antenna and, as a result, multiple phase noise parameters need to be tracked. What about for a MIMO system deployed in E-band?
    \begin{itemize}
        \item The overall packaging for a LoS MIMO system operating in E-band can be much smaller and beneficial in form factor, installation, and cost.
        \item Phase noise in such a MIMO system is much easier to address given that due to the smaller distance between the antennas a single oscillator can be used for all antennas, thus, reducing the number of phase noise parameters that need to be tracked by the carrier recovery system.
        \item The more directional antennas in the E-band can potentially result in better LoS MIMO performance and ease of installation. Do we have any evidence to support this?
        \item Any other advantages for MIMO in E-band that we can discuss here and also supported through some evidence or logic?
    \end{itemize}


\vspace{+6pt}
\noindent
\uline{\emph{4.3.3.3 Application of MIMO in Millimeter Band:}} The development of MIMO technology has been largely based on the assumption of independent and identically distributed (i.i.d.) Rayleigh fading channels, where no line-of-sight path is present and a high number of multipath components is created by the surrounding environment \cite{article_MIMO_II,article_Telatar,book_3G_EVOLUITION}. Under these circumstances, it has been theoretically shown that the MIMO capacity scales linearly with the minimum number of transmit or receive antennas \cite{article_MIMO_II,article_Telatar}. Moreover, while it is widely accepted that a single LOS path is beneficial for SISO systems, since it enhances their performance with respect to multipath conditions, these results cannot be straightforwardly extended to the point-to-point MIMO case. As a matter of fact, until recently it was believed that LOS propagation limits the beneficial effects of MIMO technology since the LOS rays are linearly dependent and as such do not result throughput gains via spatial multiplexing.


\vspace{+4pt}
\noindent Some recent investigations though have proposed design methodologies in order to achieve subchannel orthogonality which is a key condition for capacity maximization in MIMO systems. The common idea behind all these approaches is to place the antenna elements sufficiently far apart so that the spatial LOS responses become unique. The optimum spacing can be worked out via simple geometrical techniques \cite{article_MIMO_LoS,Sarris-07,article_michalis}. A schematic illustration of a conventional rank-1 and optimized LOS MIMO system is given in Figure \ref{fig:los_MIMO}, where the phenomenon of subchannel orthogonality is illustrated. More specifically,
\begin{wrapfigure}{r}{0.35\textwidth}
\begin{center}
\vspace*{-20pt}
\scalebox{0.77}{\includegraphics {Figures/los_MIMO3}}
\vspace{-338pt}
\caption{Illustration of \emph{(a)} conventional and \emph{(b)} optimized MIMO systems in LOS. The former offers minimum multiplexing gain due to the high correlation between the LOS responses whereas the latter delivers orthogonal LOS subchannels.}
\vspace*{-20pt}
\label{fig:los_MIMO}
\end{center}
\end{wrapfigure}
for a MIMO systems equipped with $N_t$ transmit and $N_r$ receiver antennas, the optimum antenna spacing at the transmitter and receiver, $d_t$, and $d_r$, respectively, for a given transmitter-receiver distance $D$ and carrier wavelength $\lambda$, is given by \cite{article_MIMO_LoS}\vspace{-2pt}
\begin{align}\label{eq:antenna_spacing}
    d_td_r=\frac{\lambda D}{\text{max}(N_t, N_r)}.
\end{align}
From \eqref{eq:antenna_spacing}, it can be easily concluded that as the operating frequency increases, the optimum antenna spacing at the transmitter and receiver become smaller, leading to transceivers of smaller dimensions. Thus, compared to microwave systems, LOS MIMO technology can be more easily applied in E-band systems, since due to the smaller antenna spacing a single oscillator may be used at all the transmit and receive antennas \cite{article_HANI_phase_noise_est} and the smaller dimension of the transceiver modules eases the installation and deployment of such systems. However, to date, very little research has been carried on the transceiver design for MIMO E-band systems as outlined in the following sub sections.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%NEW SUBSUBSUBSECTION FOR THIS SECTION
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\vspace{+6pt}
\noindent
\uline{\emph{4.3.3.4 MIMO Channel Models in E-band:}} Accurate models for the MIMO channel are vital to the design of transmitters and receivers that can effectively utilize the available spectrum and achieve full spatial multiplexing and/or diversity. The original works in the field of MIMO E-band channel modeling focused mainly on channel measurement campaigns with a view to analyze the spatial-temporal characteristics of the wireless medium \cite{Ranvier-09}. At the same time, while significant work on the channel modeling of conventional MIMO systems has been reported, e.g., \cite{Karedal-08,Cheng-09,Cheng-12} and references therein, very little is still known about the modeling of millimeter wave MIMO systems. Some very preliminary results include \cite{Torkildson-10}, in which the authors consider an outdoor deployment and examine MIMO techniques for combating fading, along with an indoor link where they examine the effect of blockage. However, the results are limited to systems operating in the 60GHz band, which is significantly different from the 70/80 GHz band due to oxygen absorption \cite{wells_10}.



\vspace{+4pt}
\noindent
At this stage of the project, our main effort will be devoted to developing new and appropriate channel models which will capture the characteristics of the MIMO channel in E-band. The focus is on the modeling of temporal, spatial, and spectral characteristics of the LOS MIMO channel matrix as well as its first and second order statistics, i.e., envelope distributions and correlation statistics, respectively, for 70, 80, and 90 GHz bands. By drawing upon the vast literature on propagation modeling, we seek to extend and complement previously reported results. Of particular interest are outdoor long range propagation scenarios that correspond to wireless backhauling or enterprise communication systems. In the modeling process we will take advantage of mathematical and physical tools as well as stochastic \cite{book_Oestges_07} and geometric techniques \cite{article_Molisch_03}. Access to the high frequency facility at UCR will also enable us to thoroughly test and verify these models against measurement results, which can further improve their accuracy and applicability.

%It is available to faculty, researchers, students, and industry who require state-of-the-art design, fabrication, and testing of RF, microwave and millimeter wave devices.
%
%Some of the equipments they have at E-band (60-90GHz) are, Sources Network Analyzer up to 67GHz Waveguide and mixer components Spectrum analyzer up to 50GHz
%
%Both network and spectrum analyzer range can be extended using mixers.
%
%
%Given the limited time, it is difficult to involve someone from UCLA formally. But you can mention a collaborative relationship between me and Prof Babak Daneshrad of UCLA and Dr. Harish Rajagopalan of UCLA, which can help us for the access to their E band equipment.
%
%You can also mention our current vector signal generators (Agilent MXG N5182A) and vector signal analyzer (Agilent MXA N9020A) at UCR, which can also be used to test the MIMO phase error solutions
%
%Depending on the model complexity, we will first explore geometry-based stochastic
%channel models (GSCMs), in which the location of the scatterers is chosen stochastically
%assuming a certain density function and the model is derived from the position of the
%scatterers by applying the fundamental laws of reflection, diffraction and scattering [31].
%Given the high complexity of GSCMs, we will also work with non-geometrical stochastic
%physical models which describe paths from transmitter to receiver by statistical parameters
%only, without reference to the geometry of the physical environment. We note that
%these models ave very useful for a posteriori simulation purposes [32].
%If time allows, we intend to assess the impact of practical impairments, such as phase
%noise, which greatly deteriorate the performance of mm-wave systems by distorting the
%received signal. Hence, these impairments need to be properly modeled in a practical
%setting.
%
%As was emphasized in Section A.2.3, the area of channel modeling for mm-wave
%MIMO systems has not been properly investigated; therefore, there is very strong research
%potential into this highly interesting field with strong industrial relevance.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%NEW SUBSUBSUBSECTION FOR THIS SECTION
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\vspace{+6pt}
\noindent
\uline{\emph{4.3.3.5 Transceiver Design for Millimeter Wave MIMO Systems:}} In order to fully realize the potential of millimeter wave band, corresponding MIMO transmitters and receivers need to be designed according to the channel and impairment models in this band.

\vspace{+4pt}
\noindent
On the transmitter side, the current research in the literature has been focused on the design of array configurations for realizing the benefits offered by MIMO technology in millimeter wave links. A main characteristic of millimeter wave MIMO systems is the lack of scattering that is available at lower frequencies \cite{wells_10}. This line-of-sight nature of the signals can be combined with beamforming techniques to improve the throughput of E-band systems. In this context, we first note the important works of Sayeed and Behdad, which introduced the concept of \emph{continuous-aperture phased MIMO (CAP-MIMO)} \cite{Sayeed-10,Sayeed-11}. CAP-MIMO refers to a novel transceiver architecture that combines the elements of MIMO, continuous aperture antennas, and phased arrays to maximize the capacity of millimeter wave MIMO systems. This is achieved via a hybrid analog-digital topology, that is, a high-resolution discrete lens array to perform analog beamforming. By doing so, one can exploit both the multiplexing gains offered by conventional discrete antenna arrays, suitable for MIMO systems, as well as the high power efficiency offered by continuous aperture dish antennas. In \cite{Huang-10,Torkildson-06, Torkildson-11}, new receiver designs are proposed by grouping a large number of antennas together and forming an analog sub-array. Each one of these sub-arrays applies an analog beamformer and the signal from these arrays are combined using a digital beamformer. This two stage approach reduces the complexity associated with beamforming for MIMO receivers operating in E-band especially as the number of antennas grows large. The capacity gains of these sophisticated configurations were noticeable for both short-range indoor and long-range outdoor links. Finally, it is important to mention the proof-of-concept works in \cite{Dyadyuk-10,Sheldon-08,Sheldon-09} that have demonstrated the potential of millimeter wave MIMO. Nevertheless, these prior works rely on simplified channel models that ignore the impact of weather phenomena and environment conditions on the overall system performance. They also ignore the effects of practical impairments such as phase noise, which result in significant performance degradation \cite{Meyr-1998,article_HANI_phase_noise_est}. Moreover, the authors in \cite{Sayeed-10,Sayeed-11,Torkildson-06, Torkildson-11} address the issue of millimeter wave MIMO communications from a pure antenna theory point of view. This implies that no communication theory tools were used in order to analytically determine the performance characteristics of these configurations.


\vspace{+4pt}
\noindent On the receiver side, the main focus has been on implementing the SISO millimeter wave receiver from electronics and circuits theory points of view while assuming that due to the large available spectrum, bandwidth efficiency is not important in the design process \cite{receiver_eband-1,receiver_eband-2,receiver_eband-3}. As a result, the proposed receivers have no carrier recovery algorithms and employ lower-order differential modulations which are known to be spectrally inefficient \cite{receiver_eband-1,receiver_eband-2,receiver_eband-3}. To the best of the PIs' knowledge, there is no work that has comprehensively addressed MIMO receiver design in E-band systems.



\subsection{More Appropriate Phase Noise Models in E-band}\label{sec:eband-pn}

\textbf{Phase noise in E-band:} Phase noise has a detrimental affect on the performance of communication systems, however, its impact in E-band might be different compared to narrowband systems and potentially more severe.
    \begin{itemize}
        \item How does the large bandwidth in E-band changes our interpretation of the phase noise spectrum mask. Does it matter if the floor of the mask is lower or higher? Can we corroborate our results by comparing the BER performance of narrowband and wideband systems for two different oscillators with different masks? This can be carried out by ensuring that Lei provides Hani with a phase noise sequence for each system and then we produce BER results for each sequence.
        \item Basically the goal of the above investigation is to provide some information of what defines a good oscillator in E-band, lower mask floor or better performance near the carrier frequency?
        \item How can one address the phase noise issue? Does the traditional PLL approaches apply here? if not then what are the new signal processing schemes that need to be taken into consideration? Maybe in such setups it would be better to consider new joint coded estimation and detection algorithms.
        \item How does this affect the application of higher order modulations in E-band? can they be used? what are the limitations?
    \end{itemize}


==> MIMO.tex <==
\section{Transceiver Design for MIMO E-band Systems}\label{sec:eband-MIMO}


The development of MIMO technology has been largely based on the assumption that due to the high number of multipath components created by surrounding environment, the application of multiple antennas at the transmitter and receiver will result in multiple independent channels between the two terminals. Under these circumstances, it has been theoretically shown that the MIMO system capacity scales linearly with the minimum number of transmit or receive antennas. Moreover, while it is widely accepted that a single LOS path is beneficial for SISO systems, since it enhances their performance with respect to multipath conditions, these results cannot be straightforwardly extended to the MIMO case. As a matter of fact, until recently it was believed that LOS propagation limits the beneficial effects of MIMO technology since the LOS rays are linearly dependent and as such do not result throughput gains via spatial multiplexing (see Fig. \ref{fig:los_MIMO}).

\begin{wrapfigure}{r}{0.35\textwidth}
\begin{center}
\vspace*{-30pt}
\scalebox{0.85}{\includegraphics {Figures/los_MIMO3}}
\vspace{-415pt}
\caption{Illustration of \emph{(a)} conventional and \emph{(b)} optimized MIMO systems in LOS. The former offers minimum multiplexing gain due to the high correlation between the LOS responses whereas the latter delivers orthogonal LOS subchannels.}
\vspace*{-20pt}
\label{fig:los_MIMO}
\end{center}
\end{wrapfigure}


Some recent investigations though have proposed design methodologies in order to achieve subchannel orthogonality. The common idea behind all these approaches is to place the antenna elements sufficiently far apart so that the spatial LOS responses become unique. The optimum spacing can be worked out via simple geometrical techniques \cite{article_MIMO_LoS}. A schematic illustration of a conventional and optimized LOS MIMO system is given in Figure \ref{fig:los_MIMO}, where the phenomenon of subchannel orthogonality is illustrated. More specifically, for a MIMO systems the optimum antenna spacing at the transmitter and receiver for a given transmitter-receiver distance is inversely proportional to the carrier frequency. Consequently, as the operating frequency increases, the optimum antenna spacing at the transmitter and receiver become smaller, leading to transceivers of smaller dimensions. Thus, compared to microwave systems, LOS MIMO technology can be more easily applied in E-band systems, since due to the smaller antenna spacing the transceiver can be housed within a compact module that can be more easily installed and deployed. However, to fully realize the potential of MIMO E-band systems, the corresponding transceiver needs to be designed according to the channel and impairment models in this band.





On the transmitter side, the current research in the literature has been focused on the design of array configurations for realizing the benefits offered by MIMO technology in E-band. The LOS nature of the signals in E-band can be combined with beamforming techniques to improve the throughput of E-band systems. In this context, we first note the concept of \emph{continuous-aperture phased MIMO (CAP-MIMO)} \cite{Sayeed-10,Sayeed-11}. CAP-MIMO refers to a novel transceiver architecture that combines the elements of MIMO, continuous aperture antennas, and phased arrays to maximize the capacity of millimeter wave MIMO systems. This is achieved via a hybrid analog-digital topology, that is, a high-resolution discrete lens array to perform analog beamforming. By doing so, one can exploit both the multiplexing gains offered by conventional discrete antenna arrays, suitable for MIMO systems, as well as the high power efficiency offered by continuous aperture dish antennas. In \cite{Huang-10,Torkildson-06, Torkildson-11}, new receiver designs are proposed by grouping a large number of antennas together and forming an analog sub-array. Each one of these sub-arrays applies an analog beamformer and the signal from these arrays are combined using a digital beamformer. This two stage approach reduces the complexity associated with beamforming for MIMO receivers operating in E-band especially as the number of antennas grows large. The capacity gains of these sophisticated configurations were noticeable for both short-range indoor and long-range outdoor links. Finally, it is important to mention the proof-of-concept works in \cite{Dyadyuk-10,Sheldon-08,Sheldon-09} that have demonstrated the potential of millimeter wave MIMO. Nevertheless, these prior works rely on simplified channel models that ignore the impact of weather phenomena and environment conditions on the overall system performance. They also ignore the effects of practical impairments such as phase noise, which can result in significant performance degradation.


\vspace{+4pt}
\noindent On the receiver side, the main focus has been on implementing the SISO millimeter wave receiver from electronics and circuits theory points of view while assuming that due to the large available spectrum, bandwidth efficiency is not important in the design process \cite{receiver_eband-1,receiver_eband-2}. As a result, the proposed receivers have no carrier recovery algorithms and employ lower-order differential modulations which are known to be spectrally inefficient \cite{receiver_eband-1,receiver_eband-2}.

\begin{figure}[t]
\begin{center}
\vspace*{-5pt}
\scalebox{0.60}{\includegraphics {Figures/radio_unit2}}
\vspace{-100pt}
\caption{Radio unit for an E-band system.}
\vspace*{-10pt}
\label{fig:radio}
\end{center}
\end{figure}


\textbf{THIS IS WHAT WE HAVE RIGHT NOW FOR MIMO TRANSCEIVER DESIGN (Notes for Michalis and Akbar):}
\begin{itemize}
    \item What has been done in the literature is not as important but we need to some how to present some results that shows from our point of view what research direction is more promising.
    \item We need some simulation results that compares the existing schemes. Do you have anything on this?
    \item Also an important contribution could be a block diagram for a transceiver based on our knowledge or based on some work that is done that shows what an E-band transceiver would end up looking like (see Fig. \ref{fig:radio}).
    \item It is also important to note that because of the E-band signals' large bandwidth, these systems require a very high sampling rate and the application of high speed digital signal processing units at the receiver. As a result, E-band systems can be more expensive to manufacture. Thus, any new receiver designs that can reduce the required sampling rate, e.g., through the elimination of the intermediate frequency (IF) stage at the receiver, would greatly facilitate the deployment of E-band wireless communication systems. Moreover, in order to effectively utilize the large bandwidth in E-band, communication systems operating in this band may require the application of advanced physical layer designs to deal with the frequency selectivity of the channel, e.g., orthogonal frequency division multiplexing (OFDM) for point-to-point wireless links and orthogonal frequency division multiple access (OFDMA) for multiple access wireless networks.
\end{itemize}




